DAD-3DHeads: A Large-scale Dense, Accurate and Diverse Dataset for 3D Head Alignment from a Single Image

We present DAD-3DHeads, a dense and diverse large-scale dataset, and a robust model for 3D Dense Head Alignment in the wild. It contains annotations of over 3.5K landmarks that accurately represent 3D head shape compared to the ground-truth scans. The data-driven model, DAD-3DNet, trained on our dataset, learns shape, expression, and pose parameters, and performs 3D reconstruction of a FLAME mesh. The model also incorporates a landmark prediction branch to take advantage of rich supervision and co-training of multiple related tasks. Experimentally, DAD-3DNet outperforms or is comparable to the state-of-the-art models in (i) 3D Head Pose Estimation on AFLW2000-3D and BIWI, (ii) 3D Face Shape Reconstruction on NoW and Feng, and (iii) 3D Dense Head Alignment and 3D Landmarks Estimation on DAD-3DHeads dataset. Finally, the diversity of DAD-3DHeads in camera angles, facial expressions, and occlusions enables a benchmark to study in-the-wild generalization and robustness to distribution shifts. The dataset webpage is https://p.farm/research/dad-3dheads.

==> tabs/2d_landmarks_datasets.tex <==
\begin{table}[h]
\footnotesize
\renewcommand{\arraystretch}{0.95}
\centering
\begin{tabular}{r|r|r|l|l}
\noalign{\smallskip}
Dataset & \#Train & \#Test & Landmarks & Vis. lmks\\
\hline
Multi-PIE \cite{Multi-PIE} & 750,000 & - & 68 &  \cmark\\
300W \cite{sagonas2013300, sagonas2016300} & 3,837 & 600 & 68 & - \\
COFW \cite{BurgosArtizzu2013RobustFL} & 1,345 & 507 & 29 & -\\
COFW-68 \cite{DBLP:journals/corr/GhiasiF15} & 1,345 & 507 & 68 & - \\
AFLW \cite{koestinger11a} & 20,000 & 4386 & 21 & - \\
AFLW-19 \cite{AFLW19} & 20,000 & 4386 & 19 & - \\
AFLW-68 \cite{AFLW68} & 20,000 & 4386 & 68 & - \\
WFLW \cite{wayne2018lab} & 7,500 & 2500 & 98 &  - \\
MERL-RAV \cite{MERL-RAV} & 15,449 & 3865 & 68 & - \\
FaceSynthetics \cite{wood2021fake} & 100,000 & - & 70 & \cmark\\
\noalign{\smallskip}
\end{tabular}
\caption{2D Facial Landmarks Datasets}
\label{t:2dlandmark_datasets}
\end{table}

==> tabs/3d_landmarks_datasets.tex <==
% \begin{table}[h]
% \footnotesize
% \renewcommand{\arraystretch}{0.95}
% \centering
% \begin{tabular}{r|c|l}
% \noalign{\smallskip}
% Dataset & Images & Landmarks\\
% \hline
% AFLW2000-3D \cite{AFLW2000-3D} & 2000 & 68\\
% BIWI dataset \cite{BIWI} & 15000 & 6918\\
% \noalign{\smallskip}
% \end{tabular}
% \caption{3D Facial Landmarks Datasets}
% \label{t:3dlandmark_datasets}
% \end{table}

\begin{table}[h]
\footnotesize
\renewcommand{\arraystretch}{0.95}
\centering
\begin{tabular}{r|c|l}
\noalign{\smallskip}
Dataset & Images\\
\hline
FaceScape \cite{FaceScape} & 18,760\\
\noalign{\smallskip}
\end{tabular}
\caption{3D Facial Datasets}
\label{t:3dlandmark_datasets}
\end{table}

18,760 textured 3D faces, captured from 938 subjects and each with 20 specific expressions

==> tabs/all_categories.tex <==
\begin{table}[t]
\footnotesize
\caption{\textbf{DAD-3DNet} performance breakdown to different annotation labels:}
\setlength{\tabcolsep}{3pt}
	\begin{subtable}[t]{.99\linewidth}\centering
		{\input{tabs/pose_dad3dnet}}	
	\end{subtable}
	\hfill
	\begin{subtable}[t]{.99\linewidth}\centering
		{\input{tabs/expression_dad3dnet}}	
	\end{subtable}
	\hfill
	\begin{subtable}[t]{.99\linewidth}\centering
		{\input{tabs/occlusion_dad3dnet}}	
	\end{subtable}
	\hfill
	\begin{subtable}[t]{.99\linewidth}\centering
		{\input{tabs/light_dad3dnet}}	
	\end{subtable}
	\hfill
	\begin{subtable}[t]{.99\linewidth}\centering
		{\input{tabs/quality_dad3dnet}}	
	\end{subtable}
% 	\vspace{1em}
\vspace{-2.0em}
\label{t:all_categories}
\end{table}
\hspace{2em}
